Importance-Aware Data Augmentation for Document-Level Neural Machine Translation

Document-level neural machine translation (DocNMT) aims to generate translations that are both coherent and cohesive, in contrast to its sentence-level counterpart. However, due to its longer input length and limited availability of training data, DocNMT often faces the challenge of data sparsity. To overcome this issue, we propose a novel Importance-Aware Data Augmentation (IADA) algorithm for DocNMT that augments the training data based on token importance information estimated by the norm of hidden states and training gradients. We conduct comprehensive experiments on three widely-used DocNMT benchmarks. Our empirical results show that our proposed IADA outperforms strong DocNMT baselines as well as several data augmentation approaches, with statistical significance on both sentence-level and document-level BLEU.

==> tables/2_preliminary.tex <==
\section{Preliminary: How to best perturb Input and Output Sequences in \docnmt?}
\label{preliminary}
In this section, we will explore the optimal strategy to perturb input and output sequences in \docnmt. Specifically, we conduct a synthetic experiment that trains a \docnmt model to memorize mappings between random number sequences. To simulate the \docnmt scenario, as shown in Figure, both input and output sequences have context number sequence and target number sequence. A sub-sequence of context number sequence is highly correlated with the input sequence, while the rest of context number sequence are generated randomly. During evaluation, we feed some of the training instance back to the model and test if the model can memorize the random output sequence given the inputs.
